Line Emission from Stellar Winds in Active Galactic Nuclei

This dissertation presents synthetic spectra and response functions of the red giant stellar line emission model of active galactic nuclei. Our results agree with the fundamental line emission characteristics of active galactic nuclei within the model uncertainties if the following additional assumptions are made: 1) the mean stellar mass loss rates decrease with distance from the black hole, and 2) the mean ionization parameters are lower than those postulated in Kazanas (1989). For models with enhanced mass loss, the zero-intensity-full-widths of the line profiles are proportional to the black hole mass to the power of 1/3. This scaling relation suggests that the black hole masses of NLS1s (narrow-line Seyfert 1s) are relatively low. Models with enhanced mass loss also predict minimum line/continuum delays that are proportional to the zero-intensity-full-widths of the profiles. Because of their high column densities, these models yield triangle-shaped response functions, which are not generally observed. On the other hand, models without enhanced mass loss yield line-continuum delays that are proportional to the square root of the continuum luminosity, which is constant with empirical results. Models with high enough intercloud (interstellar) medium densities and a BLR-occulting accretion disk have line shifts. The broadest line emission and absorption profile components of lines similar to C IV, N V, and O VI are redshifted. Conversely, the narrowest emission and absorption profile components are blueshifted in such models. These results appear to agree with observations (e.g., Done & Krolik 1996).

==> preface.tex <==
This dissertation presents results of the stellar wind line emission
model of active galactic nuclei.  These results are summarized in
Chapter
\ref{summaryanddiscussion}.  

Some of this work has been published previously in {\it Reverberation
Mapping of the Broad-Line Region in Active Galactic Nuclei} (Taylor
1994).  Portions of Appendix C were published in {\it The Astrophysical
Journal Letters} (Taylor 1998).  Results shown in Appendices F, G, and
H were published in {\it The Astrophysical Journal} (Taylor 1996).  A
version of Appendix K was submitted in May 1997 as part of a proposal
in collaboration with Demosthenes Kazanas and Mark Voit.  A version of
Appendix L was published on the World Wide Web in 1996.  

This version of the dissertation was formatted to conserve whitespace.
A black and white copy of the original version without the phrase or
author indexes is available from UMI Dissertation Services in Ann
Arbor, Michigan.
%Permission is granted to reproduce this dissertation for
%educational purposes.  
%  This version of the dissertation has been printed for the 
%University of Maryland.  A more complete and compact version of the
%dissertation will be made available by the author.


==> scriptsusedtoproduceindexes/addindextags <==
#!/bin/tcsh

# 8/21/1999 JAT 
# messy but should work
#
if ( $#argv <= 0 ) then
  echo '' 
  echo '   Usage:'; echo ''
  echo '     '$0' <file prefix>'
  echo '     Creates latex file <file>-with-index.tex with index entries of phrases in '
  echo '     indexphraselist.txt' ; echo ''
  exit 1
endif
#

echo Creating files with index tags called $1-with-index.tex ...
setenv num_of_phrases `wc indexphraselist.txt | awk '{print $1}'`
if ( $num_of_phrases <= 0 ) then
  echo Didn\'t read file.  Quitting now.
  exit 1
endif
setenv linenumber 1
# DON'T COPY SYMBOLIC LINKS---CONVERT TO REAL STOCK!!!!!:
 dos2unix -n $1.tex $1-with-index.tex   
# DON'T USE: \cp $1.tex $1-with-index.tex   
# Take care of sed bug:
 echo ' ' >> $1-with-index.tex   
# Take care of ampersands (will restore them later at end of script):
 \mv $1-with-index.tex $1-with-index-temp.tex
 cat $1-with-index-temp.tex | sed "s/\\&/ampersand/g" > $1-with-index.tex   

while ( $linenumber <= $num_of_phrases )
 setenv line `sed -n "$linenumber,$linenumber"p indexphraselist.txt`
 echo Input line is \`\`$line\'\'.
 set phrase=(`echo $line | awk -F\; '{print $1}'`)

 # The following lines eliminates many problems with labels getting messed up, but 
 # ignores skips over phrases that are at the end of the line (fix if nec.):
  setenv iwordsminus1 `expr $#phrase - 1`
  if ( `echo $line | \grep ' ;'` != "" ) set phrase= ( ${phrase[-$iwordsminus1]} ${phrase[$#phrase]}' ' )

 set indexphrase=(`echo $line | awk -F\; '{print $2}'`)
 if ( "$indexphrase" == "" ) set indexphrase=($phrase)

 echo Matching phrase:$phrase.  Index phrase:$indexphrase

 # find out how many words are in the phrase 
 echo Total of $#phrase words in phrase.
 setenv i2 1
 while ( $i2 <= $#phrase ) 
  echo Now doing word number $i2, which is\ ${phrase[$i2]}.
   \mv $1-with-index.tex $1-with-index-temp.tex
   if ( $i2 == 1 ) then 
    setenv tail ''
    cat $1-with-index-temp.tex | sed "s/$phrase$tail/$phrase\\index\{$indexphrase\}/g" > $1-with-index.tex
   else 
    setenv i2minus1 `expr $i2 - 1`
    echo beg of phrase = ${phrase[-$i2minus1]}, end of phrase = ${phrase[$i2-]}.
    cat $1-with-index-temp.tex | sed "/${phrase[-$i2minus1]}/N;s/${phrase[-$i2minus1]}\n${phrase[$i2-]}/$phrase\\index\{$indexphrase\}%\\
/g" > $1-with-index.tex
    #      /Microsoft[ \t]*$/{ 
    #                             N 
    #                             }
    #     /Microsoft[ \t\n]*Windows[ \t]*$/{ 
    #                             N 
    #                             }
    #     s/Microsoft[ \t\n]*Windows[ \t\n]*95/Linux/g
    # cat $1-with-index-temp.tex | sed "N;s/${phrase[-$i2minus1]}\n${phrase[$i2-]}[ ]/$phrase\\index\{$indexphrase\}\\
    #/g" > $1-with-index.tex
    endif
    \rm $1-with-index-temp.tex
    setenv i2 `expr $i2 + 1`
 end
 setenv linenumber `expr $linenumber + 1`
end

\mv $1-with-index.tex $1-with-index-temp.tex
cat $1-with-index-temp.tex | sed "s/ampersand/\\\&/g"  > $1-with-index.tex   
\rm $1-with-index-temp.tex


==> scriptsusedtoproduceindexes/cleanupauthorindexfile <==
#
echo '\\par ~' >! $1.bib
cat $1.ind | \grep -v '{theindex}' | \grep -v '\indexspace' | sed 's/\\bf,/\\bf~ /g' | sed 's/\\bf  ,/\\bf~ /g' | sed 's/\\bf ,/\\bf~ /g' | sed 's/\\item/\\par \\rm/g' >> $1.bib
echo '\\rm' >> $1.bib


==> scriptsusedtoproduceindexes/phrasecounter <==
#!/usr/bin/perl -w
use strict;
my $n = shift @ARGV;
die "usage: $0 nwords [input]\n" if not defined ($n) or $n == 0;
my %phrases;
my @phrase;

while (<>) {
	my @line = split;
	for (@line) {
		push @phrase, $_;  # add next word
		# cut and pasted -- ick, sorry
		$phrases{join ' ', @phrase} ++ if @phrase == $n;
		if (@phrase == $n + 1) {
			shift @phrase;  # remove oldest word
			$phrases{join ' ', @phrase} ++;
		}
	}
}

print map { sprintf ("%8d %s\n", $phrases{$_}, $_) } 
	sort { $phrases{$b} <=> $phrases{$a} } 
	keys %phrases;


==> scriptsusedtoproduceindexes/removespacesinauthoridxfile <==
#

cat $1.idx | sed 's/\\bf  \}/\\bf\} /g'  >! $1-temp.idx
\mv $1-temp.idx $1.idx


==> scriptsusedtoproduceindexes/runeverything <==
#
set verbose
mkdir tmp
\mv -f a.tex tmp/
cat thesischapter1.tex thesischapter2and3.tex thesischapter4.tex thesischapter5.tex thesisextra.tex > a.tex
emacs a.tex -batch -l ~/.emacs -f 'parselyx' -f 'save-buffer'
unalias a
\mv -f indexphraselist.txt backup.txt
ln -s indexphraselist-authors.txt indexphraselist.txt 
runaddindextags |\grep Creating
   # Needs a clean slate to avoid index indexing itself and simple scripts:
   \mv -f a-with-index.bib a-with-index-last.bib  ; touch a-with-index.bib  
   \mv -f a-with-index.ind a-with-index-last.ind  ; touch a-with-index.ind 
makesourcereadable # run this only if source needs to be clean:
\latex a-with-index
\latex a-with-index
\latex a-with-index
removespacesinauthoridxfile a-with-index
makeindex a-with-index
cleanupauthorindexfile a-with-index
   \mv -f a-with-index.bib a-with-index-temp.bib ; touch a-with-index.bib 
   \rm a-with-index.ind  ; touch a-with-index.ind 

alias makeclean '\mv -f \!*\-with-index.tex tmp/\!*\-with-index-phrase.tex'
makeclean a
makeclean adpbal
makeclean darkma
makeclean shiftsap
makeclean td1small
makeclean td2small
makeclean td1small-tbl
makeclean veldtemp

\rm indexphraselist.txt 
ln -s indexphraselist-phrases.txt indexphraselist.txt 
runaddindextags |\grep Creating 
makesourcereadable # run this only if source needs to be clean:
\latex a-with-index
\latex a-with-index
\latex a-with-index
makeindex a-with-index
   \rm a-with-index.bib 
   \mv a-with-index-temp.bib a-with-index.bib
alias makeclean '\mv -f \!*\-with-index.tex tmp/\!*\-with-index-author.tex; cp \!*.tex \!*\-with-index.tex'
makeclean a
makeclean adpbal
makeclean darkma
makeclean shiftsap
makeclean td1small
makeclean td2small
makeclean td1small-tbl
makeclean veldtemp
\latex a-with-index
\latex a-with-index
prepare-a.texforvtex
dvips a-with-index
ps2pdf a-with-index.ps a-with-index.pdf
unset verbose
echo 'Now all you need to do is reboot into windows and compile to html.'

